Illumination Estimation Challenge: experience of past two years

Illumination estimation is the essential step of computational color constancy, one of the core parts of various image processing pipelines of modern digital cameras. Having an accurate and reliable illumination estimation is important for reducing the illumination influence on the image colors. To motivate the generation of new ideas and the development of new algorithms in this field, the 2nd Illumination estimation challenge~(IEC\#2) was conducted. The main advantage of testing a method on a challenge over testing in on some of the known datasets is the fact that the ground-truth illuminations for the challenge test images are unknown up until the results have been submitted, which prevents any potential hyperparameter tuning that may be biased. The challenge had several tracks: general, indoor, and two-illuminant with each of them focusing on different parameters of the scenes. Other main features of it are a new large dataset of images (about 5000) taken with the same camera sensor model, a manual markup accompanying each image, diverse content with scenes taken in numerous countries under a huge variety of illuminations extracted by using the SpyderCube calibration object, and a contest-like markup for the images from the Cube+ dataset that was used in IEC\#1. This paper focuses on the description of the past two challenges, algorithms which won in each track, and the conclusions that were drawn based on the results obtained during the 1st and 2nd challenge that can be useful for similar future developments.

==> chapters/4_results_overview.tex <==
\subsection{Challenge results}
\label{subsec:tracksresults}

\subsubsection{General track results.}
\label{subsubsec:generalresult}

\begin{table*}[ht]
\normalsize
\caption{General track leadboard}
\label{tab:general_leader}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Team & Algorithm & \textbf{Mean (worst 25\%)} & Mean & Median & Trimean \\
\hline
\hline
\textcolor{gold}{\textbf{Z. Li}} & \textcolor{gold}{\textbf{CAUnet (sub. \# ?)}} & \textcolor{gold}{4.084077} & \textcolor{gold}{1.605}  & \textcolor{gold}{0.966} & \textcolor{gold}{1.084} \\
\hline
\textbf{Z. Li} & \textbf{CAUnet  (sub. \# ?)} & 4.321251 & 1.725  & 1.084 & 1.207 \\
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 4.419051 & 1.822  & 1.197 & 1.317 \\
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 4.656795 & 1.891  & 1.230 & 1.352 \\
\hline
\textcolor{silver}{\textbf{Y. Qian}} & \textcolor{silver}{\textbf{sde-awb (sub. \# ?)}} & \textcolor{silver}{4.979334} & \textcolor{silver}{1.914} & \textcolor{silver}{1.164} & \textcolor{silver}{1.269} \\
\hline
\textbf{Y. Qian} & \textbf{sde-awb (sub. \# ?)} & 5.112188 & 1.952 & 1.149 & 1.292 \\
\hline
\textbf{Y. Qian} & \textbf{sde-awb (sub. \# ?)} &  5.377026 & 2.034 & 1.150 & 1.282\\
\hline
\textbf{J. Qiu et al.} & \textbf{illumGAN} & 9.999407 & 4.643 & 3.588 & 3.841 \\
\hline
IITP BASELINE & \textbf{GreyWorld} & 10.419472 & 4.500 & 3.319 & 3.611 \\
\hline
IITP BASELINE & \textbf{Constant} & 17.023748 & 7.081 & 4.020 & 5.275\\
\hline
\textcolor{bronze}{\textbf{J. Qiu et al.}} & \textcolor{bronze}{\textbf{illGAN1.0 (sub. \# ?)}} &  \textcolor{bronze}{25.954709} & \textcolor{bronze}{19.325} & \textcolor{bronze}{18.278} & \textcolor{bronze}{18.499}\\
\hline
\textbf{J. Qiu et al.} & \textbf{illGAN1.0 (sub. \# ?)} & 26.058358 & 19.360 & 18.328 & 18.498 \\
\hline
\textbf{J. Qiu et al.} & \textbf{illGAN1.0 (sub. \# ?)} & 26.459121 & 19.408 & 18.468 & 18.710 \\
\hline
\end{tabular}
\end{table*}
The first place was achieved by Z. Li (Nanjing University) with CAUnet algorithm. 
Final mean reproduction error for 25\% of the worst images was 4.084077 for this algorithm.


\subsubsection{Indoor track results.}
\label{subsubsec:indoorresult}

\begin{table*}[ht]
\normalsize
\caption{Indoor track leadboard}
\label{tab:indoor_leader}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    Team & Algorithm & \textbf{Mean} & Median & Trimean \\
\hline
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 2.500120 & 2.293 & 2.201 \\
\hline
\textcolor{gold}{\textbf{Y. Qian}} & \textcolor{gold}{\textbf{sde-awb}} & \textcolor{gold}{2.541370} & \textcolor{gold}{1.763} & \textcolor{gold}{1.943} \\
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 2.855412 & 2.293 & 2.407 \\
\hline
\textbf{J. Qiu et al.} & \textbf{illumGAN} & 3.191023 & 2.596 & 2.674 \\
\hline
\textcolor{silver}{\textbf{R. Riva et al.}} & \textcolor{silver}{\textbf{PCGAN, MCGAN (sub. \# ?)}} & \textcolor{silver}{3.301088} & \textcolor{silver}{2.312} & \textcolor{silver}{2.298} \\
\hline
\textbf{R. Riva et al.} & \textbf{PCGAN, MCGAN (sub. \# ?)} & 3.376422 & 2.312 & 2.337 \\ 
\hline
IITP BASELINE & \textbf{GreyWorld} & 4.105811 & 3.673 & 3.545 \\
\hline
IITP BASELINE & \textbf{Constant} & 15.269933 & 14.802 & 15.332 \\ 
\hline
\end{tabular}
\end{table*}

The first place was achieved by Y. Qian (Huawei MultiMedia Team) with sde-awb algorithm. 
Final mean reproduction error was 2.541370 for this algorithm.



\subsubsection{Two-illuminant track results.}
\label{subsubsec:twoilluminantresult}

\begin{table*}[ht]
\normalsize
\caption{Two-illuminant track leadboard}
\label{tab:twoilluminant_leader}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Team & Algorithm & \textbf{Mean squared} & Mean & Median & Trimean \\
\hline
\hline
\textcolor{gold}{\textbf{Y. Qian}} & \textcolor{gold}{\textbf{sde-awb (sub. \# ?)}} & \textcolor{gold}{31.026217} & \textcolor{gold}{2.751} & \textcolor{gold}{2.262} & \textcolor{gold}{2.290} \\
\hline
\textbf{Y. Qian} & \textbf{sde-awb (sub. \# ?)} & 31.542930 & 2.737 & 2.171 & 2.309 \\ 
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 33.079119 & 2.657 & 1.844 & 2.082 \\
\hline
\textbf{Y. Liu et al.} & \textbf{3du-awb} & 37.305135 & 2.863 & 2.503 & 2.497 \\
\hline
\textbf{X. Xing et al.} & \textbf{AL-AWB (sub. \# ?)} & 41.883269 & 2.920 & 2.107 & 2.316 \\
\hline
IITP BASELINE & \textbf{GreyWorld} & 81.840743 & 4.127 & 3.538 & 3.715 \\
\hline
IITP BASELINE & \textbf{Constant} & 144.745182 & 5.264 & 3.475 & 3.815 \\ 
\hline
\end{tabular}
\end{table*}

The first place was achieved by Y. Qian (Huawei MultiMedia Team) with sde-awb algorithm. 
Final squared sum of two angular reproduction errors was 31.026217 for this algorithm.





==> chapters/5_method_description.tex <==
\section{Method description}
\label{sec:methods}

\subsection{CAUnet}

% TODO: picture
% TODO: full description

\subsection{PCGAN, MCGAN}

% TODO: picture
% TODO: full description

\subsection{AL-AWB}

% TODO: picture
% TODO: full description

==> chapters/7_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

% TODO

==> chapters/bio.tex <==
\section*{Biography}
% bio approx 3 sentences, ORCID for submitting author
\hspace{0.5cm}\textbf{Egor Ershov} (ORCID=\url{https://orcid.org/0000-0001-6797-6284})
received a Ph.D. degree from the Faculty of Radio Engineering and Computer Technology in 2019. 
He is a senior researcher in Vision System Laboratory in Institute of Information Transmission Problems (Kharkevic Institute) of the Russian Academy of science (IITP RAS).
He is also senior lecturer at Computer Science Faculty in Higher School of Economy.
His main areas of research are image processing and analysis, particularly color computer vision, color reproduction technologies, colorimetry, human vision system, Hough transform.
He is an assistance manager of the cathedra at Computer Science faculty in Higher School of Economy.
He is a recipient of several awards for his scientific and professional work.

\textbf{Alex (Alexey) Savchik} 
Vision  Systems  Laboratory,  Institute   for   Information   Transmission   Problems (Kharkevich Institute) of the Russian Academy of Sciences (IITP RAS), Moscow, Russia. 
Alex Savchik in 2014 graduated from Department of Mechanics and Mathematics of Moscow State Univercity, in 2012 from Yandex School of Data Analysis. His research interests include deep learning and computer vision.

\textbf{Ilya (Illya) Semenkov} Vision  Systems  Laboratory,  Institute   for   Information   Transmission   Problems (Kharkevich Institute) of the Russian Academy of Sciences (IITP RAS), Moscow, Russia. 
Received Bachelor's degree at National Research University Higher School of Economics (NRU HSE) in 2019 and is currently Master's student at Faculty of Computer Science of NRU HSE. 
His research interests include Deep Learning, Computer Vision, Statistical Learning and Optimal Transport. 

\textbf{Arseniy Terekhin} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Daria Senshina} Vision  Systems  Laboratory,  Institute   for   Information   Transmission   Problems (Kharkevich Institute) of the Russian Academy of Sciences (IITP RAS), Moscow, Russia. 
Received Bachelor's degree at Moscow Institute of Physics and Technology (MIPT) in 2020. 
Daria Senshina is currently Master's student at Phystech School of Applied Mathematics and Informatics of MIPT and simultaneously obtaining M.Sc. degree in Industrial and Applied Maths at the University Grenoble Alpes, Grenoble, France. 
Her research interests include computer vision and image processing.

\textbf{Artem Nikonorov (b. 1979).} He received his Candidate and Doctor of Sciences degree in 2005 and 2016. Now he works as a head of AI Center of the Samara University and head of Video Intelligence Lab of the Image Processing Systems Institute of RAS. He has more than 80 publications, two monographs. Scope of scientific interest: pattern recognition and image analysis, machine learning, computational imaging, parallel and distributed programming. E-mail: artniko@gmail.com .

\textbf{Dmitry Nikolaev} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Nikola Bani{\'{c}}} received B.Sc., M.Sc., and Ph.D. degrees in computer science in 2011, 2013, and 2016, respectively. 
He is currently working as a senior computer vision engineer at Gideon Brothers, Croatia. 
He has worked in real-time image enhancement for embedded systems, digital signature recognition, people tracking and counting, and image processing for stereo vision. 
His research interests include image enhancement, color constancy, image processing for stereo vision, and tone mapping.

\textbf{Karlo Ko{\v{s}}{\v{c}}evi{\'{c}}} received B.Sc. and M.Sc. degrees in computer science in 2016 and 2018, respectively. 
He is currently in his second year of the technical sciences in the scientific field of computing Ph.D. program at the Faculty of Electrical Engineering and Computing, University of Zagreb, Croatia. 
His research interests include image processing, image analysis, and deep learning. 
His current research is in the area of color constancy with a focus on learning-based methods for illumination estimation.

\textbf{Marko Suba{\v{s}}i{\'{c}}} received a Ph.D. degree from the Faculty of Electrical Engineering and Computing at the University of Zagreb in 2007. 
Since 1999, he has been working at the Department for Electronic Systems and Information Processing at the Faculty of Electrical Engineering and Computing at the University of Zagreb, currently as an associate professor. 
He teaches several courses at the graduate and undergraduate levels. 
His research interests lie in image processing and analysis and neural networks, with a particular interest in image segmentation, detection techniques, and deep learning. 
He is a member of the IEEE - Computer Society, the Croatian Center for Computer Vision, the Croatian Society for Biomedical Engineering and Medical Physics, and the Centre of Research Excellence for Data Science and Advanced Cooperative Systems. 

\textbf{Sven Lon{\v{c}}ari{\'{c}}} received B.Sc., M.Sc., and Ph.D. degrees in 1985, 1989, and 1994, respectively. 
After earning his doctoral degree, he continued his academic career at the Faculty of Electrical Engineering and Computing, University of Zagreb, where he is currently a full professor. 
He was an assistant professor at the Department of Electrical and Computer Engineering, New Jersey Institute of Technology, NJ, USA, from 2001-2003. 
His main areas of research are image processing and analysis. 
Together with his students and collaborators, he has published more than 200 publications in scientific peer-reviewed journals and has presented his work at international conferences. 
He is a senior member of the IEEE, director of the Center for Artificial Intelligence, and co-director of the national Center of Research Excellence for Data Science and Advanced Cooperative Systems. 
He is a recipient of several awards for his scientific and professional work.

\textbf{Marco Buzzelli} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Riccardo Riva} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Simone Bianco} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Raimondo Schettini} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Zhihao Li} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

\textbf{Yanlin Qian} is a well-known author in the field of the journal scope. His/Her research interests include interest 1, interest 2.\par

